Unconditional Quantile Partial Effects via Conditional Quantile Regression

This paper develops a semi-parametric procedure for estimation of unconditional quantile partial effects using quantile regression coefficients. The estimator is based on an identification result showing that, for continuous covariates, unconditional quantile effects are a weighted average of conditional ones at particular quantile levels that depend on the covariates. We propose a two-step estimator for the unconditional effects where in the first step one estimates a structural quantile regression model, and in the second step a nonparametric regression is applied to the first step coefficients. We establish the asymptotic properties of the estimator, say consistency and asymptotic normality. Monte Carlo simulations show numerical evidence that the estimator has very good finite sample performance and is robust to the selection of bandwidth and kernel. To illustrate the proposed method, we study the canonical application of the Engel's curve, i.e. food expenditures as a share of income.

==> Engel_Curves.tex <==


A New Engel on Price Index and Welfare Estimation
David Atkin, Benjamin Faber, Thibault Fally, and Marco Gonzalez-Navarro
NBER Working Paper No. 26890
March 2020

Omitted Variable Bias in Engel Curve Estimation

The first issue is common to all Engel curve estimates: if household taste differences are correlated with household income, Engel curves will be biased. For example, more educated households may both value certain goods more and have higher incomes. This would bias our price
index and welfare estimates, as changes in real income over time would not affect budget shares
in the way our estimated Engel curves predict. This bias can be addressed either by controlling
for household characteristics in the estimation of relative Engel curves or by estimating curves
separately for different types of household (both of which we pursue in Section 6).

An Engel Curve for Variety 
Nicholas Li
Author and Article Information
The Review of Economics and Statistics (2021) 103 (1): 72–87.

Uses IV

IZA DP No. 15674
Gains from Trade and the Food Engel
Curve
Farid Farrokhi
David Jinkins
Chong Xiang
OCTOBER 2022
https://docs.iza.org/dp15674.pdf

Identification and Estimation of Engel Curves with Endogenous and Unobserved Expenditures
Erich Battistin, Michele De Nadai
First published: 18 September 2013 https://doi.org/10.1002/jae.2349Citations: 7
Read the full text
PDFPDFTOOLS SHARE
Summary
When dealing with the estimation of Engel curves, measurement errors in expenditure data and simultaneity are likely sources of endogeneity. In this paper we study identification of the parameters that characterize an Engel curve in the presence of both. We consider specifications where budget shares are polynomials in the logarithm of total expenditure, which is the case frequently encountered in empirical applications. We propose an estimation procedure which is an extension of that in Lewbel (1996) and exploits a control function assumption to correct for the endogeneity of the true unobserved total expenditure.

The Review of Economics and Statistics
Vol. XCIII November 2011 Number 4
A TEST OF CONSPICUOUS CONSUMPTION: VISIBILITY AND
INCOME ELASTICITIES
Ori Heffetz*
Abstract—This paper shows that, consistent with a signaling-by-consuming
model à la Veblen, income elasticities can be predicted from the visibility
of consumer expenditures. We outline a stylized conspicuous consumption
model where income elasticity is endogenously predicted to be higher if a
good is visible and lower if it is not. We then develop a survey-based measure
of expenditure visibility, ranking different expenditures by how noticeable
they are to others. Finally, we show that our visibility measure predicts
up to one-third of the observed variation in elasticities across consumption
categories in U.S. data.

Charles, Kerwin, Erik Hurst, and Nikolai Roussanov, “Conspicuous Consumption and Race,” Quarterly Journal of Economics 124 (2009),
425–467.
https://www.nber.org/papers/w13392

The table reports the coefficient on the race dummies from a regression of the log
of visible consumption on a race dummies and other controls. Specification 2 includes the log of current income, if income is positive, a cubic in the level of
current income, and a dummy for whether current income was positive. Specification 3 also includes the log of total expenditure, and a cubic in the level of total
expenditure. Specification 4 is the same as specification 3 without the income controls. Specification 5 is the same as specification 3 but also includes three
education dummies (exactly high school, some college, or college or more). Specification 6 includes year dummies. Specification 7 also includes a quadratic in
age, a male dummy, a married dummy, census regions dummies, a MSA dummy, an urban dummy, wealth controls, and a series of separate dummies for the
number of adults and children in the household


The Journal of Socio-Economics
Volume 45, August 2013, Pages 146-154
The Journal of Socio-Economics
A test of the conspicuous–consumption model using subjective well-being data☆
Author links open overlay panelRicardo Perez-Truglia
